A Note on the Hausdorff Number of Compact Topological Spaces

The notion of Hausdorff number of a topological space is first introduced in \cite{bonan}, with the main objective of using this notion to obtain generalizations of some known bounds for cardinality of topological spaces. Here we consider this notion from a topological point of view and examine interrelations of the Hausdorff number with compactness.

==> Bibliography.bib.tex <==
%Bibliography

%
%
%
%  TOPOLOGY  AND  SET  THEORY
%
%
%


@article{Shafaat,
author= {Lucio R. Berrone},
title={On the Number Topologies Definable for a Finite Set},
journal = "Journal of the Australian Mathematical Society",
year ="1968",
volume ="8",
number ="2",
pages ="194-198"
month ="",
note = {},
key=""
}

@article{benoumhani,
author= {Lucio R. Berrone},
title={On the Number of Finite Topological Spaces},
journal = "Le Matematiche",
year ="1993",
volume ="XLVIII",
number ="1",
pages ="87-99"
month ="",
note = {},
key=""
}


@article{benoumhani,
author= {Moussa Benoumhani},
title={The {N}umber of Topologies on a Finite Set },
journal = "Journal of Integer Sequences",
year ="2006",
volume ="9",
number ="",
pages =""
month ="",
note = {},
key=""
}


@article{Stong,
author= {R. E. Stong},
title={Finite {T}opological {S}paces },
journal = "Transactions of the American Mathematical Society",
year ="1966",
volume ="123",
number ="2",
pages ="325-340"
month ="",
note = {},
key=""
}

@article{Bonan,
author= {Maddalena Bonanzinga},
title={On the {H}ausdorff {N}umber of a {T}opological {S}pace },
journal = "Houston Journal of Mathematics",
year ="2005",
volume ="76",
number ="1",
pages =""
month ="",
note = {},
key=""
}

@article{Lind,
author= {Ernst L. {Lindel\"of}},
title={Sur quelques points de la th\'eorie des ensembles},
year="1903",
journal = "C. R. Acad. Paris",
volume="137",
pages="697-700"
}%reference from Engelking

@article{AU,
author={Pavel Alexandroff and Pavel Urysohn},
title={M\'emoire sur les espaces topologiques compacts},
year={1929},
journal={Verh. Akad. Wetensch. Amsterdam},
volume={14},
number={},
pages={}
} %reference from Engelking

@article{Fro,
author={Z. Frolik},
title={Generalizations of compact and Lindel\"of spaces},
year={1959},
journal={Czech. Math. J.},
volume={9},
number={},
page={172-217}
}

@proceedings{J,
author="Istvan Juhasz",
title="Hereditarily Almost {Lindel\"of} Spaces",
publisher="Presented at the International Topological Conference, Varna, Bulgaria",
year="1991"
}

@article{Sorg,
author="Robert H. Sorgenfrey",
title="On the topological product of paracompact spaces",
year="1947",
journal=" Bull. Amer. Math. Soc.",
volume="53",
pages="631-632"
}%reference from Engelking

@book{SW,
author="Stephen Willard",
title="General Topology",
year="2004",
publisher="Dover Publications, INC.",
}

@book{ENG,
author="Ryszard Engelking",
title="General Topology",
publisher="Heldermann",
edition="Revised and completed",
year="1989"
}

@book{SDb,
author="Sheldon Davis",
title="Topology",
publisher="McGraw-Hill Science/Engineering/Math",
edition="First",
year={2004},
}

@book{SS,
author="Lynn A. Steen and J. Arthur Seebach",
title="Counterexamples in {T}opology",
publisher="Dover Publications Inc.",
edition="New",
year="1996"
}

@article{CS,
author={F. Cammaroto and G. Santoro},
title={Some counterexamples and properties on generalizations of Lindel\"of spaces},
year={1996},
journal={Internat. J. Math. {\&} Math. Sci.},
volume={19},
number={4},
page={737-746}
}

@article{DW,
author={S. Willard and U. N. B. Dissanayake},
title={The almost Lindel\"of degree},
year={1984},
journal={Canad. Math. Bull.},
volume={27},
number={4},
page={452-455}
}

@article{SZ,
author={Y. Song and Y. Zhang},
title={Some remarks on almost {L}indel\"of spaces and weakly {L}indel\"of spaces},
year={2010},
journal={Matematicheskii Vestnik},
volume={62},
number={},
page={77-83}
}

@article{HJ,
author={A. Hajnal and I. Juhasz},
title={On the products of weakly Lindel\"of spaces},
year={1975},
journal={Proceedings of the American Mathematical Society},
volume={48},
number={2},
page={454-456},
note={%\url{http://www.jstor.org/stable/2040282}
}
}

@article{Bon,
author={D. Bonnett},
title={A symmetrizable space that is not perfect},
year={1972},
journal={Proceedings of the American Mathematical Society},
volume={34},
number={2},
page={560-564}
}

@article{M,
author={A. Mysior},
title={A regular space which is not completely regular},
year={1981},
journal={Proceedings of the American Mathematical Society},
volume={81},
number={4},
page={652-653}
}

@article{Win,
author={R. Winkler},
title={A simple Hausdorff space which is Lindel\"of, first countable, CCC but not separable},
year={1996},
journal={Anzeiger Abt.},
volume={II},
number={133},
page={23-25},
note={%\url{http://hw.oeaw.ac.at/0xc1aa500d_0x000221d0.pdf}
}
}

@article{BGW,
author={M. Bell and J. Ginsburg and G. Woods},
title={Cardinal inequalities for topological spaces involving the weak Lindel\"of number},
year={1978},
journal={Pacific Journal of Mathematics},
volume={79},
number={1},
page={37-45},
note={%\url{http://projecteuclid.org/DPubS/Repository/1.0/Disseminate?view=body&id=pdf_1&handle=euclid.pjm/1102805984}
}
}

@MISC{Henno,
  author = {Henno Brandsmal},
  title = {{CCC} implies separable},
  month = Feb,
  year = {2011},
  howpublished={[online resource]},
  note = "\url{http://at.yorku.ca/cgi-bin/bbqa?forum=ask_a_topologist;task=show_msg;msg=1977}"
}

@MISC{SxS,
  author = {J. Mashburn},
  title = {Homework Solutions},
  howpublished={[online resource]},
  note = "\url{http://academic.udayton.edu/joemashburn/471/homework/solutions/homework6.pdf}"
}

@article{Stav,
author={S. Davis and D. Stavrova},
title={Covering properties of symmetrizable spaces},
year={2009},
journal={Comptes rendus de l'Acad\'emie bulgare des Sciences},
volume={62},
number={8},
page={923-928},
note={\url{http://www.proceedings.bas.bg/}}
}

@article{A,
author={A. Archangelskii},
title={A theorem on cardinality},
year={1979},
journal={Russ. Math. Surv.},
volume={34},
number={153},
page={},
note={%\url{http://iopscience.iop.org/0036-0279/34/4/L06;jsessionid=2F37EA196DEA8274B5C185043A8E3346.c1}
}
}
@MISC{B1b,
  author = { Robin {Dr Knight}},
  title = {B1b Set Theory Lecture Notes},
  howpublished={[online resource]},
  note = "\url{http://www.maths.ox.ac.uk/courses/course/12440/material}"
}@MISC{Topology,
  author = {Dr. Drutu},
  title = {Part A Topology Lecture Notes},
  howpublished={[online resource]},
  note = "\url{http://www.maths.ox.ac.uk/courses/course/12513/material}"
}@MISC{PartC,
  author = {},
  title = {C1.2a Analytic Topology Lecture Notes},
  howpublished={[online resource]},
  note = "\url{http://www.maths.ox.ac.uk/courses/course/12461}"
}


%
%
%
%  NUMBER THEORY
%
%
%


@book{Wald5,
author= {Michael Waldschmidt},
title={Nombres transcendants},
year="1974",
publisher = "Springer-Verlag",
volume="402",
series = "Lecture Notes in Mathematics",
address ="Berlin"
}

@misc{waldschmidtslides1,
author= {Michael Waldschmidt},
title = {Some Consequences of {S}chanuel's Conjecture},
howpublished = {\url{http://www.math.jussieu.fr/~miw/articles/pdf/AWSProject2.pdf}},
note={Online Beamer Presentation}
}

@article{Nesterenko2,
author= {Yurii Nesterenko},
title={On the number {$\pi$} and {L}indemann's Theorem},
journal = "Commentationes Mathematicae Universitatis Carolinae",
year ="1979",
volume ="20",
number ="2",
pages ="335-343"
month ="",
note = {\url{http://dml.cz/dmlcz/105932}},
key=""
}

@misc{Butler,
author= {Lee Butler},
title = {Transcendence and Irrationality Proofs},
howpublished = {\url{http://www.maths.bris.ac.uk/~malab/PDFs/MA469.pdf}},
note="Fourth year project"
}

@article{Baker1,
author= {Alan Baker},
title={Linear forms in the logarithms of algebraic numbers. {I}. },
year="1966",
journal = "Mathematika. A Journal of Pure and Applied Mathematics",
volume="13",
number = "",
pages="204-216"
}

@article{Baker2,
author= {Alan Baker},
title={Linear forms in the logarithms of algebraic numbers. {II}. {III}.},
year="1967",
journal = "Mathematika. A Journal of Pure and Applied Mathematics",
volume="14",
number = "",
pages="102-107,220-228"
}

@article{Schneider,
author= {Theodor Schneider},
title={Transzendenzuntersuchungen periodischer {F}unktionen. {I}. {II}.},
year="1934",
journal = "J. Reine Angew. Math.",
volume="172",
number = "",
pages="65-69,70-74"
}


@article{Lin,
author= {F.-C. Lin},
title={Schanuel's Conjecture implies {R}itt's Conjecture},
year="1983",
journal = "Chinese J. Math",
issue = "11",
pages="41-50",
note=""
}



@misc{WaldSC2009,
author={Michael Waldschmidt},
title={Schanuel's {C}onjecture and {C}riteria for {A}lgebraic {I}ndependence},
note={Online Beamer Presentation},
howpublished = "\url{http://www.math.jussieu.fr/~miw/articles/pdf/SchanuelConjecture2009.pdf}"
}

@misc{SCVariants,
author= {Jonathan Kirby},
title={Variants of {S}chanuel's {C}onjecture},
year="2007",
month = "Sept",
note="Expository article",
howpublished = {\url{http://www.uea.ac.uk/~ccf09tku/pdf/SCvariants.pdf}}
}

@article{Lindemann,
author= {Carl Louis Ferdinand von Lindemann},
title={{\"U}ber die {L}udolph'sche {Z}ahl},
year="1882",
journal = "Sitzungsberichte der Akademie der Wiss. Berlin",
volume="2",
issue = "",
pages="679-682",
note=""
}




@article{Nesterenko,
author= {Yurii Nesterenko},
title={Modular functions and transcendence questions},
year="1996",
journal = "Mat. Sb",
volume="187",
issue = "9",
pages="65-96"
}

@article{Sondow,
author= {Jonathan Sondow and Diego Marques},
title={Schanuel's {C}onjecture and algebraic powers {$z^w$} and {$w^z$} with {$z$} and {$w$} transcendental},
year="2010",
journal = "East-West Journal of Mathematics",
volume="12",
number = "1",
pages="75-84"
}

@book{Goldrei,
author= "Derek Goldrei",
title={Classic Set Theory For Guided Independent Study},
year="1996",
publisher="Chapman \& Hall",
volume="",
edition="1st",
address = ""
}

@article{Weierstrass,
author= {K. Weierstra{\ss}},
title={Zu {L}indemann's {A}bhandlung ``\"{U}ber die {L}udolph'sche {Z}ahl{"}},
year="1885",
journal = "Sitzungsber. Preu{\ss}. Akad. Wiss. zu Berlin",
volume="2",
number = "",
pages="1067-1085"
}

@article{Beukers,
author= {Frits Beukers and {Jean-Paul} Bezivin and Philippe Robba},
title={An {A}lternative {P}roof of the {L}indemann-{W}eierstra{\ss} {T}heorem},
year="1990",
journal = "The American Mathematical Monthly",
volume="97",
number = "3",
pages="193-197"
}

@article{Kirbypaper,
author= {Jonathan Kirby},
title={Exponential algebraicity in exponential fields},
year="2010",
journal = "Bulletin of the  London Mathematical Society",
volume="42",
number = "5",
pages="879-890"
}

@article{Zilber2,
author= {Boris Zilber},
title={Exponential sums equations and the {S}chanuel conjecture},
year="2002",
journal = "Journal of the London Mathematical Society",
volume="65",
issue = "2",
pages="27-44"
}

@article{vDMM,
author= {L. van den Dries and Angus Macintyre and David Marker},
title={On the elementary theory of restricted analytic functions with exponentiation},
year="1994",
journal = "Annals of Math.",
volume="140",
issue = "",
pages="183-205"
}

@book{MarkerModelTh,
author= "David Marker",
title={Model Theory: an Introduction},
year="2002",
publisher="Springer-Verlag",
volume="",
address = "New York"
}

@book{MW,
author= {Angus Macintyre and Alex Wilkie},
title={On the decidability of the real exponential field},
booktitle={Kreisel 70th Birthday Volume},
editor={P. G. Odifreddi},
year="1995",
journal = "",
volume="",
issue = "",
number="CLSI",
pages="59-90"
}

@misc{ZilberDay,
author= {Boris Zilber},
title={On transcendental number theory, classical analytic functions and {D}iophantine geometry},
howpublished ="\url{http://www.phil.uu.nl/~iemhoff/Beauty/ZilberDay.pdf}",
note ="Online resource"
}

@misc{Kirby,
  author = {Jonathan Kirby},
  title = {Complex {E}xponentiation and {Z}ilber's {P}seudo-exponentiation},
  month = {Apr},
  year = {2009},
  howpublished={\url{http://at.yorku.ca/cgi-bin/bbqa?forum=ask_a_topologist;task=show_msg;msg=1977}},
  note = {Online Resource}
}

@article{Marker,
author= {David Marker},
title={A remark on {Z}ilber's pseudoexponentiation},
year="2006",
journal = "Journal of Symbolic Logic",
volume="71",
issue = "3",
pages="791-798"
}

@incollection{SurveysNumberTheory,
editor = "Krishnaswami Alladi",
author = "Michael Waldschmidt",
title={Surveys in Number Theory},
year="2008",
publisher="Springer",
edition="1st",
address = "",
booktitle = "Developments in Mathematics"
}

@article{Schneider6exp,
author= {Theodor Schneider},
title={Ein Satz \"{u}ber ganzwertige Funktionen als Prinzip f\"{u}r Transzendenzbeweise},
year="1949",
journal = "Math. Ann.",
volume="121",
number = "",
pages="131-140"
}


@article{AlaogluErdos,
author= { L. Alaoglu\ and\ P. Erd\"os},
title={On highly composite and similar numbers},
year="1944",
journal = "Trans. Amer. Math. Soc.",
volume="56",
number = "",
pages="448-469"
}

@article{Wald2,
author= {Michael Waldschmidt},
title={Fonctions auxiliaires et fonctionnelles analytiques. {I}, {II},},
year="1991",
journal = "J. Analyse Math.",
volume="56",
number = "",
pages="231-254,255-279"
}


@book{Eulersqrt2,
author= "Leonhard Euler",
title={Introduction in {A}nalysin {I}nfinitorum. ({O}pera {O}mnia. {S}eries {P}rima: {O}pera {M}athematica,)},
year="1945",
publisher="Societas Scientiarum Naturalium Helveticae",
volume="Volumen Novum",
address = "Geneva"
}



@article{Gelfond,
author= "Aleksandr Gel'fond",
title={Sur le septi\'eme probl\'eme de {D}. {H}ilbert},
year="1934",
journal = "Izv. Akad. Nauk SSSR",
volume="7",
number = "",
pages="623-630"
}

@article{waldAuxFn,
author= "Michael Waldschmidt",
title={Auxiliary functions in transcendental number theory},
year="2009",
journal = "The Ramanujan journal",
volume="20",
number = "3",
pages="341-373"
}

@article{winterschool,
author= "Chuangxun Cheng and Brian Dietel and Mathilde Herblot and Jingjing Huang and Holly Krieger and Diego Marques and Jonathan Mason and Martin Mereb and S Robert Wilson",
title={Some consequences of Schanuel's Conjecture},
year="2008",
journal = "Arizona Winter School 2008",
volume="",
number = "",
pages=""
}

@article{Zilber,
author= {Boris Zilber},
title={Pseudo-exponentiation on algebraically closed fields of characteristic zero},
year="2005",
journal = "Annals of Pure and Applied Logic",
volume="132",
number = "1",
pages="67-95"
}

@article{Terzo,
author= {Guiseppina Terzo},
title={Some Consequences of {S}chanuel's {C}onjecture in exponential rings},
year="2008",
journal = "Communications in Algebra",
volume="36",
number = "",
pages="1171-1189"
}


@book{Rama,
author="Kanakanahalli Ramachandra",
title="Contributions to the theory of transcendental numbers. {I}, {II}",
year="1967/1968",
publisher="Acta Arith.",
pages="73-88"
}

@book{Lang,
author="Serge Lang",
title="Introduction to Transcendental numbers",
year="1966",
publisher="Addison-Wesley Publishing Co",
%Reading, Massachussets
}

@book{Rose,
author="H. E. Rose",
title="A Course in Number Theory",
year="1994",
publisher="Oxford University Press",
series = "Oxford Science Publications",
}

@book{WaldBook,
author="Michael Waldschmidt",
title="Diophantine approximation on linear algebraic groups. Transcendence properties of the exponential function in several variables",
year = "2000",
publisher="Springer-Verlag Berlin",
series="Grundlehren der Mathematischens Wissenschaften [Fundamental Principles of Mathematical Sciences]"
}


@book{NumberFriends,
author="Paulo Ribenboim",
title="My Numbers, My Friends: Popular Lectures on Number Theory",
year="2000",
publisher="Springer-Verlag New York, Inc",
}


@article{Chow,
author= {Timothy Chow},
title={What is a {C}losed-{F}orm {N}umber?},
year="1999",
journal = "The American Mathematical Monthly",
volume="106",
number = "5",
pages="440-448"
}

@book{MTT,
author = "Edward Burger and Robert Tubbs",
title = "Making Transcendence Transparent",
year = "2004",
publisher="Springer Science Business Media Inc",
}

@book{Niven,
author="Ivan Niven",
title="The Carus Mathematical Monographs",
year="1956",
publisher="The Mathematical Association of America",
edition = "second"
}


@book{Baker,
author="Alan Baker",
title="Transcendental Number Theory",
year="1990",
publisher="Cambridge University Press",
}


@book{100GP,
author="Heinrich {D\"orrie}",
title="100 Great Problems of Elementary Mathematics",
year="1965",
publisher="Dover Publications Inc",
}

@article{Hermite,
author= {Charles Hermite},
title={Sur la fonction exponentielle},
year="1873",
journal = "Compte Rendu Academie Scientifique",
volume="77",
pages="18-24"
}%reference from Engelking



%
%
%
% OTHER
%
%
%

@book{Priestley,
author= "Hilary Priestley",
title={Introduction to Complex Analysis},
year="2004",
publisher="Oxford University Press",
edition ="2nd",
series = ""
}

@book{LangAlgebra,
author= "Serge Lang",
title={Algebra},
year="2002",
publisher="Springer",
edition ="3d",
series = "Graduate Texts in Mathematics"
}
